Antenna Array Design for Mono-Static ISAC

Mono-static sensing operations in ISAC perform joint beamforming between transmitter and receiver. However, in contrast to pure radar systems, ISAC requires to fulfill communications tasks and to retain the corresponding design constraints for at least one half-duplex antenna array. This shifts the available degrees of freedom to the design of the second half-duplex array, that completes the mono-static sensing setup of the 6G ISAC system. Consequently, although it is still possible to achieve the gains foreseen by the radar sparse array literature, it is necessary to adapt these considerations to the new ISAC paradigm. In this work, we propose a model to evaluate the angular capabilities of a mono-static setup, constrained to the shape of the communications array and its topology requirements in wireless networks. Accordingly, we enhance the joint angular capabilities by utilizing a sparse element topology of the sensing array with the same number of elements. Our analysis is validated by simulation experiments, confirming the value of our model in providing system designers with a tool to drastically improve the trade-off between angular capabilities for sensing and the cost of the deployed hardware.

==> Figures/Prob_MD/prob_md_0dB.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\def\scale{.72}

\begin{semilogyaxis}[
    xlabel={$\Delta d^{(\text{P})}$},
    ylabel={$P^\text{(MD)}$},
    ylabel shift = -14 pt,
    ylabel style={font=\footnotesize,at={(axis description cs:.-0.05,.5)},rotate=0,anchor=south},
    ytick={0.00001, 0.00002, 0.00003, 0.00004, 0.00005, 0.00006, 0.00007, 0.00008, 0.00009, 0.0001, 0.0002, 0.0003, 0.0004, 0.0005, 0.0006, 0.0007, 0.0008, 0.0009, 0.001, 0.002, 0.003, 0.004, 0.005, 0.006, 0.007, 0.008, 0.009, 0.01, 0.02, 0.03, 0.04, 0.05, 0.06, 0.07, 0.08, 0.09, 0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 1, 2, 3, 4, 5, 6},
    yticklabels={$10^{-5}$, , , , , , , , ,$10^{-4}$, , , , , , , , ,$10^{-3}$, , , , , , , , ,$10^{-2}$, , , , , , , , , , , , , , , , , , $10^{0}$},
    xlabel style={font=\footnotesize},
    yticklabel style={font=\footnotesize,xshift=3pt},
    xticklabel style={
        /pgf/number format/precision=4,
        /pgf/number format/fixed, 
        font=\footnotesize},
    ymin=1e-2,
    ymax=1e-0,
    xmin=0.02,
    xmax=0.16,
    scaled x ticks = false,
    minor tick num=1,
    yminorticks = true,
    enlargelimits = false,
    legend pos = south west,
    grid = both,
    grid style={solid, black!15},
    legend columns = 3,
    %transpose legend,
%    		legend style={at={(0.4,0.5)}, font=\scriptsize},
    legend style={
    cells={anchor=west},
    draw=none,
    fill=none,
    }
%		xticklabels = {$1 \cdot 10^{-3}$, ,$2 \cdot 10^{-3}$,},
    % tick label style={/pgf/number format/fixed},
%        ticklabel style={font=\footnotesize},
    % legend cell align={left},
    every axis plot/.append style={very thick},
    mark repeat={2},
    log origin y=infty,
    set layers=Bowpark,
    % legend to name = common_legend,
    scale = \scale
]

% % common legend
% \addplot[very thick, color=violet, solid, draw=none] coordinates {(0, 1)}; \addlegendentry{\(\square^{(\text{S})} = 3\times3\)}
% \addplot[very thick, color=teal, solid, draw=none] coordinates {(0, 1)}; \addlegendentry{\(\square^{(\text{S})} = 5\times5\)}
% \addplot[very thick, color=cyan, solid, draw=none] coordinates {(0, 1)}; \addlegendentry{\(\square^{(\text{S})} = 7\times7\)}
% \addplot[very thick, color=black, solid, draw=none] coordinates {(0, 1)}; \addlegendentry{\(d^{(\text{S})} /\lambda = 0.5 \;\)}
% \addplot[very thick, color=black, dashed, draw=none] coordinates {(0, 1)}; \addlegendentry{\(d^{(\text{S})} /\lambda = 1.5 \;\)}
% \addplot[very thick, color=black, dotted, draw=none] coordinates {(0, 1)};\addlegendentry{\(d^{(\text{S})} /\lambda = 2.0\)}

\def\noise{"0"}

\def\sensshape{"3"}
\def\sensspacing{"0.5"}
\addplot [very thick, violet, solid] plot table[x index=0, y index=1] {Data/Prob_MD/prob_md_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};
\def\sensspacing{"1.5"}
\addplot [very thick, violet, dashed] plot table[x index=0, y index=1] {Data/Prob_MD/prob_md_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};
\def\sensspacing{"2.0"}
\addplot [very thick, violet, dotted] plot table[x index=0, y index=1] {Data/Prob_MD/prob_md_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};

\def\sensshape{"5"}
\def\sensspacing{"0.5"}
\addplot [very thick, teal, solid] plot table[x index=0, y index=1] {Data/Prob_MD/prob_md_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};
\def\sensspacing{"1.5"}
\addplot [very thick, teal, dashed] plot table[x index=0, y index=1] {Data/Prob_MD/prob_md_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};
\def\sensspacing{"2.0"}
\addplot [very thick, teal, dotted] plot table[x index=0, y index=1] {Data/Prob_MD/prob_md_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};

\def\sensshape{"7"}
\def\sensspacing{"0.5"}
\addplot [very thick, cyan, solid] plot table[x index=0, y index=1] {Data/Prob_MD/prob_md_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};
\def\sensspacing{"1.5"}
\addplot [very thick, cyan, dashed] plot table[x index=0, y index=1] {Data/Prob_MD/prob_md_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};
\def\sensspacing{"2.0"}
\addplot [very thick, cyan, dotted] plot table[x index=0, y index=1] {Data/Prob_MD/prob_md_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};

\end{semilogyaxis}

\end{tikzpicture}


==> Figures/Prob_MD/prob_md_10dB.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\def\scale{.72}

\begin{semilogyaxis}[
    xlabel={$\Delta d^{(\text{P})}$},
    ylabel={$P^\text{(MD)}$},
    ylabel shift = -14 pt,
    ylabel style={font=\footnotesize,at={(axis description cs:.-0.05,.5)},rotate=0,anchor=south},
    ytick={0.00001, 0.00002, 0.00003, 0.00004, 0.00005, 0.00006, 0.00007, 0.00008, 0.00009, 0.0001, 0.0002, 0.0003, 0.0004, 0.0005, 0.0006, 0.0007, 0.0008, 0.0009, 0.001, 0.002, 0.003, 0.004, 0.005, 0.006, 0.007, 0.008, 0.009, 0.01, 0.02, 0.03, 0.04, 0.05, 0.06, 0.07, 0.08, 0.09, 0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 1, 2, 3, 4, 5, 6},
    yticklabels={$10^{-5}$, , , , , , , , ,$10^{-4}$, , , , , , , , ,$10^{-3}$, , , , , , , , ,$10^{-2}$, , , , , , , , , , , , , , , , , , $10^{0}$},
    xlabel style={font=\footnotesize},
    yticklabel style={font=\footnotesize,xshift=3pt},
    xticklabel style={
        /pgf/number format/precision=4,
        /pgf/number format/fixed, 
        font=\footnotesize},
    ymin=1e-2,
    ymax=1e-0,
    xmin=0.02,
    xmax=0.16,
    scaled x ticks = false,
    minor tick num=1,
    yminorticks = true,
    enlargelimits = false,
    legend pos = south west,
    grid = both,
    grid style={solid, black!15},
    legend columns = 3,
    %transpose legend,
%    		legend style={at={(0.4,0.5)}, font=\scriptsize},
    legend style={
    cells={anchor=west},
    draw=none,
    fill=none,
    }
%		xticklabels = {$1 \cdot 10^{-3}$, ,$2 \cdot 10^{-3}$,},
    % tick label style={/pgf/number format/fixed},
%        ticklabel style={font=\footnotesize},
    % legend cell align={left},
    every axis plot/.append style={very thick},
    mark repeat={2},
    log origin y=infty,
    set layers=Bowpark,
    % legend to name = common_legend,
    scale = \scale
]

% % common legend
% \addplot[very thick, color=violet, solid, draw=none] coordinates {(0, 1)}; \addlegendentry{\(\square^{(\text{S})} = 3\times3\)}
% \addplot[very thick, color=teal, solid, draw=none] coordinates {(0, 1)}; \addlegendentry{\(\square^{(\text{S})} = 5\times5\)}
% \addplot[very thick, color=cyan, solid, draw=none] coordinates {(0, 1)}; \addlegendentry{\(\square^{(\text{S})} = 7\times7\)}
% \addplot[very thick, color=black, solid, draw=none] coordinates {(0, 1)}; \addlegendentry{\(d^{(\text{S})} /\lambda = 0.5 \;\)}
% \addplot[very thick, color=black, dashed, draw=none] coordinates {(0, 1)}; \addlegendentry{\(d^{(\text{S})} /\lambda = 1.5 \;\)}
% \addplot[very thick, color=black, dotted, draw=none] coordinates {(0, 1)};\addlegendentry{\(d^{(\text{S})} /\lambda = 2.0\)}

\def\noise{"10"}

\def\sensshape{"3"}
\def\sensspacing{"0.5"}
\addplot [very thick, violet, solid]  plot table[x index=0, y index=1] {Data/Prob_MD/prob_md_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};
\def\sensspacing{"1.5"}
\addplot [very thick, violet, dashed] plot table[x index=0, y index=1] {Data/Prob_MD/prob_md_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};
\def\sensspacing{"2.0"}
\addplot [very thick, violet, dotted] plot table[x index=0, y index=1] {Data/Prob_MD/prob_md_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};

\def\sensshape{"5"}
\def\sensspacing{"0.5"}
\addplot [very thick, teal, solid] plot table[x index=0, y index=1] {Data/Prob_MD/prob_md_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};
\def\sensspacing{"1.5"}
\addplot [very thick, teal, dashed] plot table[x index=0, y index=1] {Data/Prob_MD/prob_md_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};
\def\sensspacing{"2.0"}
\addplot [very thick, teal, dotted] plot table[x index=0, y index=1] {Data/Prob_MD/prob_md_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};

\def\sensshape{"7"}
\def\sensspacing{"0.5"}
\addplot [very thick, cyan, solid] plot table[x index=0, y index=1] {Data/Prob_MD/prob_md_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};
\def\sensspacing{"1.5"}
\addplot [very thick, cyan, dashed] plot table[x index=0, y index=1] {Data/Prob_MD/prob_md_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};
\def\sensspacing{"2.0"}
\addplot [very thick, cyan, dotted] plot table[x index=0, y index=1] {Data/Prob_MD/prob_md_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};

\end{semilogyaxis}

\end{tikzpicture}


==> Figures/RMSE1st/rmse_1st_-10dB.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\def\scale{.72}

\begin{semilogyaxis}[
    xlabel={$\Delta d^{(\text{P})}$},
    ylabel={\gls{naf} \gls{rmse}},
    ylabel shift = -14 pt,
    ylabel style={font=\footnotesize,at={(axis description cs:.-0.05,.5)},rotate=0,anchor=south},
    ytick={0.00001, 0.00002, 0.00003, 0.00004, 0.00005, 0.00006, 0.00007, 0.00008, 0.00009, 0.0001, 0.0002, 0.0003, 0.0004, 0.0005, 0.0006, 0.0007, 0.0008, 0.0009, 0.001, 0.002, 0.003, 0.004, 0.005, 0.006, 0.007, 0.008, 0.009, 0.01, 0.02, 0.03, 0.04, 0.05, 0.06, 0.07, 0.08, 0.09, 0.1, 0.2},
    yticklabels={$10^{-5}$, , , , , , , , ,$10^{-4}$, , , , , , , , ,$10^{-3}$, , , , , , , , , , , , , , , , , ,$10^{-1}$, , , , , , , , , $10^{0}$},
    xlabel style={font=\footnotesize},
    yticklabel style={font=\footnotesize,xshift=3pt},
    xticklabel style={
        /pgf/number format/precision=4,
        /pgf/number format/fixed, 
        font=\footnotesize},
    ymin=1e-3,
    ymax=1e-1,
    xmin=0.02,
    xmax=0.16,
    scaled x ticks = false,
    minor tick num=1,
    yminorticks = true,
    enlargelimits = false,
    legend pos = south west,
    grid = both,
    grid style={solid, black!15},
    legend columns = 3,
    %transpose legend,
%    		legend style={at={(0.4,0.5)}, font=\scriptsize},
    legend style={
    cells={anchor=west},
    draw=none,
    fill=none,
    }
%		xticklabels = {$1 \cdot 10^{-3}$, ,$2 \cdot 10^{-3}$,},
    % tick label style={/pgf/number format/fixed},
%        ticklabel style={font=\footnotesize},
    % legend cell align={left},
    every axis plot/.append style={very thick},
    mark repeat={2},
    log origin y=infty,
    set layers=Bowpark,
    % legend to name = common_legend,
    scale = \scale
]

% % common legend
% \addplot[very thick, color=violet, solid, draw=none] coordinates {(0, 1)}; \addlegendentry{\(\square^{(\text{S})} = 3\times3\)}
% \addplot[very thick, color=teal, solid, draw=none] coordinates {(0, 1)}; \addlegendentry{\(\square^{(\text{S})} = 5\times5\)}
% \addplot[very thick, color=cyan, solid, draw=none] coordinates {(0, 1)}; \addlegendentry{\(\square^{(\text{S})} = 7\times7\)}
% \addplot[very thick, color=black, solid, draw=none] coordinates {(0, 1)}; \addlegendentry{\(d^{(\text{S})} /\lambda = 0.5 \;\)}
% \addplot[very thick, color=black, dashed, draw=none] coordinates {(0, 1)}; \addlegendentry{\(d^{(\text{S})} /\lambda = 1.5 \;\)}
% \addplot[very thick, color=black, dotted, draw=none] coordinates {(0, 1)};\addlegendentry{\(d^{(\text{S})} /\lambda = 2.0\)}

\def\noise{"-10"}

\def\sensshape{"3"}
\def\sensspacing{"0.5"}
\addplot [very thick, violet, solid] plot table[x index=0, y index=1] {Data/RMSE1st/rmse_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};
\def\sensspacing{"1.5"}
\addplot [very thick, violet, dashed] plot table[x index=0, y index=1] {Data/RMSE1st/rmse_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};
\def\sensspacing{"2.0"}
\addplot [very thick, violet, dotted] plot table[x index=0, y index=1] {Data/RMSE1st/rmse_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};

\def\sensshape{"5"}
\def\sensspacing{"0.5"}
\addplot [very thick, teal, solid] plot table[x index=0, y index=1] {Data/RMSE1st/rmse_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};
\def\sensspacing{"1.5"}
\addplot [very thick, teal, dashed] plot table[x index=0, y index=1] {Data/RMSE1st/rmse_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};
\def\sensspacing{"2.0"}
\addplot [very thick, teal, dotted] plot table[x index=0, y index=1] {Data/RMSE1st/rmse_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};

\def\sensshape{"7"}
\def\sensspacing{"0.5"}
\addplot [very thick, cyan, solid] plot table[x index=0, y index=1] {Data/RMSE1st/rmse_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};
\def\sensspacing{"1.5"}
\addplot [very thick, cyan, dashed] plot table[x index=0, y index=1] {Data/RMSE1st/rmse_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};
\def\sensspacing{"2.0"}
\addplot [very thick, cyan, dotted] plot table[x index=0, y index=1] {Data/RMSE1st/rmse_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};

\end{semilogyaxis}

\end{tikzpicture}


==> Figures/RMSE1st/rmse_1st_0dB.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\def\scale{.72}

\begin{semilogyaxis}[
    xlabel={$\Delta d^{(\text{P})}$},
    ylabel={\gls{naf} \gls{rmse}},
    ylabel shift = -14 pt,
    ylabel style={font=\footnotesize,at={(axis description cs:.-0.05,.5)},rotate=0,anchor=south},
    ytick={0.00001, 0.00002, 0.00003, 0.00004, 0.00005, 0.00006, 0.00007, 0.00008, 0.00009, 0.0001, 0.0002, 0.0003, 0.0004, 0.0005, 0.0006, 0.0007, 0.0008, 0.0009, 0.001, 0.002, 0.003, 0.004, 0.005, 0.006, 0.007, 0.008, 0.009, 0.01, 0.02, 0.03, 0.04, 0.05, 0.06, 0.07, 0.08, 0.09, 0.1, 0.2},
    yticklabels={$10^{-5}$, , , , , , , , ,$10^{-4}$, , , , , , , , ,$10^{-3}$, , , , , , , , , , , , , , , , , ,$10^{-1}$, , , , , , , , , $10^{0}$},
    xlabel style={font=\footnotesize},
    yticklabel style={font=\footnotesize,xshift=3pt},
    xticklabel style={
        /pgf/number format/precision=4,
        /pgf/number format/fixed, 
        font=\footnotesize},
    ymin=1e-3,
    ymax=1e-1,
    xmin=0.02,
    xmax=0.16,
    scaled x ticks = false,
    minor tick num=1,
    yminorticks = true,
    enlargelimits = false,
    legend pos = south west,
    grid = both,
    grid style={solid, black!15},
    legend columns = 3,
    %transpose legend,
%    		legend style={at={(0.4,0.5)}, font=\scriptsize},
    legend style={
    cells={anchor=west},
    draw=none,
    fill=none,
    }
%		xticklabels = {$1 \cdot 10^{-3}$, ,$2 \cdot 10^{-3}$,},
    % tick label style={/pgf/number format/fixed},
%        ticklabel style={font=\footnotesize},
    % legend cell align={left},
    every axis plot/.append style={very thick},
    mark repeat={2},
    log origin y=infty,
    set layers=Bowpark,
    % legend to name = common_legend,
    scale = \scale
]

% % common legend
% \addplot[very thick, color=violet, solid, draw=none] coordinates {(0, 1)}; \addlegendentry{\(\square^{(\text{S})} = 3\times3\)}
% \addplot[very thick, color=teal, solid, draw=none] coordinates {(0, 1)}; \addlegendentry{\(\square^{(\text{S})} = 5\times5\)}
% \addplot[very thick, color=cyan, solid, draw=none] coordinates {(0, 1)}; \addlegendentry{\(\square^{(\text{S})} = 7\times7\)}
% \addplot[very thick, color=black, solid, draw=none] coordinates {(0, 1)}; \addlegendentry{\(d^{(\text{S})} /\lambda = 0.5 \;\)}
% \addplot[very thick, color=black, dashed, draw=none] coordinates {(0, 1)}; \addlegendentry{\(d^{(\text{S})} /\lambda = 1.5 \;\)}
% \addplot[very thick, color=black, dotted, draw=none] coordinates {(0, 1)};\addlegendentry{\(d^{(\text{S})} /\lambda = 2.0\)}

\def\noise{"0"}

\def\sensshape{"3"}
\def\sensspacing{"0.5"}
\addplot [very thick, violet, solid] plot table[x index=0, y index=1] {Data/RMSE1st/rmse_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};
\def\sensspacing{"1.5"}
\addplot [very thick, violet, dashed] plot table[x index=0, y index=1] {Data/RMSE1st/rmse_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};
\def\sensspacing{"2.0"}
\addplot [very thick, violet, dotted] plot table[x index=0, y index=1] {Data/RMSE1st/rmse_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};

\def\sensshape{"5"}
\def\sensspacing{"0.5"}
\addplot [very thick, teal, solid] plot table[x index=0, y index=1] {Data/RMSE1st/rmse_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};
\def\sensspacing{"1.5"}
\addplot [very thick, teal, dashed] plot table[x index=0, y index=1] {Data/RMSE1st/rmse_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};
\def\sensspacing{"2.0"}
\addplot [very thick, teal, dotted] plot table[x index=0, y index=1] {Data/RMSE1st/rmse_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};

\def\sensshape{"7"}
\def\sensspacing{"0.5"}
\addplot [very thick, cyan, solid] plot table[x index=0, y index=1] {Data/RMSE1st/rmse_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};
\def\sensspacing{"1.5"}
\addplot [very thick, cyan, dashed] plot table[x index=0, y index=1] {Data/RMSE1st/rmse_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};
\def\sensspacing{"2.0"}
\addplot [very thick, cyan, dotted] plot table[x index=0, y index=1] {Data/RMSE1st/rmse_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};

\end{semilogyaxis}

\end{tikzpicture}


==> Figures/RMSE1st/rmse_1st_10dB.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\def\scale{.72}

\begin{semilogyaxis}[
    xlabel={$\Delta d^{(\text{P})}$},
    ylabel={\gls{naf} \gls{rmse}},
    ylabel shift = -14 pt,
    ylabel style={font=\footnotesize,at={(axis description cs:.-0.05,.5)},rotate=0,anchor=south},
    ytick={0.00001, 0.00002, 0.00003, 0.00004, 0.00005, 0.00006, 0.00007, 0.00008, 0.00009, 0.0001, 0.0002, 0.0003, 0.0004, 0.0005, 0.0006, 0.0007, 0.0008, 0.0009, 0.001, 0.002, 0.003, 0.004, 0.005, 0.006, 0.007, 0.008, 0.009, 0.01, 0.02, 0.03, 0.04, 0.05, 0.06, 0.07, 0.08, 0.09, 0.1, 0.2},
    yticklabels={$10^{-5}$, , , , , , , , ,$10^{-4}$, , , , , , , , ,$10^{-3}$, , , , , , , , , , , , , , , , , ,$10^{-1}$, , , , , , , , , $10^{0}$},
    xlabel style={font=\footnotesize},
    yticklabel style={font=\footnotesize,xshift=3pt},
    xticklabel style={
        /pgf/number format/precision=4,
        /pgf/number format/fixed, 
        font=\footnotesize},
    ymin=1e-3,
    ymax=1e-1,
    xmin=0.02,
    xmax=0.16,
    scaled x ticks = false,
    minor tick num=1,
    yminorticks = true,
    enlargelimits = false,
    legend pos = south west,
    grid = both,
    grid style={solid, black!15},
    legend columns = 3,
    %transpose legend,
%    		legend style={at={(0.4,0.5)}, font=\scriptsize},
    legend style={
    cells={anchor=west},
    draw=none,
    fill=none,
    }
%		xticklabels = {$1 \cdot 10^{-3}$, ,$2 \cdot 10^{-3}$,},
    % tick label style={/pgf/number format/fixed},
%        ticklabel style={font=\footnotesize},
    % legend cell align={left},
    every axis plot/.append style={very thick},
    mark repeat={2},
    log origin y=infty,
    set layers=Bowpark,
    % legend to name = common_legend,
    scale = \scale
]

% % common legend
% \addplot[very thick, color=violet, solid, draw=none] coordinates {(0, 1)}; \addlegendentry{\(\square^{(\text{S})} = 3\times3\)}
% \addplot[very thick, color=teal, solid, draw=none] coordinates {(0, 1)}; \addlegendentry{\(\square^{(\text{S})} = 5\times5\)}
% \addplot[very thick, color=cyan, solid, draw=none] coordinates {(0, 1)}; \addlegendentry{\(\square^{(\text{S})} = 7\times7\)}
% \addplot[very thick, color=black, solid, draw=none] coordinates {(0, 1)}; \addlegendentry{\(d^{(\text{S})} /\lambda = 0.5 \;\)}
% \addplot[very thick, color=black, dashed, draw=none] coordinates {(0, 1)}; \addlegendentry{\(d^{(\text{S})} /\lambda = 1.5 \;\)}
% \addplot[very thick, color=black, dotted, draw=none] coordinates {(0, 1)};\addlegendentry{\(d^{(\text{S})} /\lambda = 2.0\)}

\def\noise{"10"}

\def\sensshape{"3"}
\def\sensspacing{"0.5"}
\addplot [very thick, violet, solid] plot table[x index=0, y index=1] {Data/RMSE1st/rmse_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};
\def\sensspacing{"1.5"}
\addplot [very thick, violet, dashed] plot table[x index=0, y index=1] {Data/RMSE1st/rmse_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};
\def\sensspacing{"2.0"}
\addplot [very thick, violet, dotted] plot table[x index=0, y index=1] {Data/RMSE1st/rmse_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};

\def\sensshape{"5"}
\def\sensspacing{"0.5"}
\addplot [very thick, teal, solid] plot table[x index=0, y index=1] {Data/RMSE1st/rmse_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};
\def\sensspacing{"1.5"}
\addplot [very thick, teal, dashed] plot table[x index=0, y index=1] {Data/RMSE1st/rmse_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};
\def\sensspacing{"2.0"}
\addplot [very thick, teal, dotted] plot table[x index=0, y index=1] {Data/RMSE1st/rmse_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};

\def\sensshape{"7"}
\def\sensspacing{"0.5"}
\addplot [very thick, cyan, solid] plot table[x index=0, y index=1] {Data/RMSE1st/rmse_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};
\def\sensspacing{"1.5"}
\addplot [very thick, cyan, dashed] plot table[x index=0, y index=1] {Data/RMSE1st/rmse_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};
\def\sensspacing{"2.0"}
\addplot [very thick, cyan, dotted] plot table[x index=0, y index=1] {Data/RMSE1st/rmse_\sensshape_by_\sensshape_d_\sensspacing_noise_\noise_dB.txt};

\end{semilogyaxis}

\end{tikzpicture}

